Neural Network Memory Architectures for Autonomous Robot Navigation

This paper highlights the significance of including memory structures in neural networks when the latter are used to learn perception-action loops for autonomous robot navigation. Traditional navigation approaches rely on global maps of the environment to overcome cul-de-sacs and plan feasible motions. Yet, maintaining an accurate global map may be challenging in real-world settings. A possible way to mitigate this limitation is to use learning techniques that forgo hand-engineered map representations and infer appropriate control responses directly from sensed information. An important but unexplored aspect of such approaches is the effect of memory on their performance. This work is a first thorough study of memory structures for deep-neural-network-based robot navigation, and offers novel tools to train such networks from supervision and quantify their ability to generalize to unseen scenarios. We analyze the separation and generalization abilities of feedforward, long short-term memory, and differentiable neural computer networks. We introduce a new method to evaluate the generalization ability by estimating the VC-dimension of networks with a final linear readout layer. We validate that the VC estimates are good predictors of actual test performance. The reported method can be applied to deep learning problems beyond robotics.

==> tex/Implementation.tex <==
\section{Implementation}
\label{sec:implementation}

We now describe our experimental setup and implementation details.

\subsection{Robot Platform}
We evaluate our approach using a grid-wold simulation. The robot state $x_t := (\mathsf{x}_t,\mathsf{y}_t)^T$ represents the 2D position of the robot. In addition there is a goal state $x_{t}^{g} := (\mathsf{x}_t^{g},\mathsf{y}_t^{g})^T$ which represents the 2D position of the goal. The robot can take 4 actions (down, right, up, left), and moves a distance of $0.5$ meters with each step. 

The robot is equipped with a laser range finder that reports the former's relative distance from any perceived obstacles that are within the laser's field of view. Let $z_{min}, z_{max}$ be the minimum and maximum range of the sensor in meters, respectively, and $N_B$ be the number of beams the sensor emits. The sensor measurement at time $t$ is $z_t := d$ where $d$ is the actual distance from the sensor to the closest obstacle along each laser beam. In our simulation we set $N_B = 1080$, $z_{min} = 0.1$ meters, and $z_{max} = 2.0$ meters. The field of view is set to $360 ^{\circ}$.

\subsection{Obstacles}
\begin{figure}[t!]
\vspace*{0.05in}
\centering
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=120px]{figures/cul-de-sac-crop-small.png}
\includegraphics[width=120px]{figures/parallel-lines-crop-small.png}
\vspace{0.1cm}
\end{subfigure}
\caption{\textbf{\textit{Left}}: Cul-de-sac \textbf{\textit{Right}}:Parallel walls. The yellow is the robot, the green is the goal region, the red is the obstacle, and the cyan is the LIDAR scan reading. In this example, the obstacle length is $10$m and the width is $3$m. The maximum LIDAR scan range is $2$m, so the robot does not know whether the obstacle is a cul-de-sac or parallel walls until it reaches the end of the obstacle.} 
\label{fig:obtacle_examples}
\vspace*{-0.15in}
\end{figure}

We use two types of obstacle courses: cul-de-sac and parallel walls (see Fig. \ref{fig:obtacle_examples}). The obstacle is either a cul-de-sac, or parallel walls. The robot does not know what type of obstacle it encounters until it reaches the end of the obstacle and sees whether there is a closed off wall or not. We use both obstacle types, instead of just the cul-de-sac, in order to ensure that the robot must learn to reach the end of the obstacle course before making a decision.

In order to generate training examples, we sample from a grid of possible parameters: obstacle length, obstacle width, obstacle orientation, start row displacement, and start column displacement. The default start position is at the beginning of the obstacle course centered in the middle of the parallel walls, and the displacement parameters shift the start location.

During our empirical test evaluation, we test for the neural network's ability to interpolate and extrapolate. We choose a grid of possible parameters for the interpolation test set, and a separate grid of parameters for the extrapolation test set. Please see Table \ref{table:map_generation_parameters} for the map generation parameters.

\begin{table}[thpb]
	\vspace*{-0.2cm}
	\begin{center} 
 		\setlength\extrarowheight{10pt}
 		\resizebox{0.48\textwidth}{!}
 		{\begin{tabular}{||c | c | c | c||} 
        \hline
 		\textbf{Parameter} & \textbf{Train} & \textbf{Interpolation Test} & \textbf{Extrapolation Test}\\ [0.6ex] 
 		\hline\hline
 		obs. length (\textit{m}) & 6, 8, 10, 12 & 7, 9, 11 & 20, 24, 28\\
 		\hline
 		obs. width (\textit{m}) & 2, 3, 4 & 2.5, 3.5 & 2.5, 3.5\\
  		\hline
 		obs. orientation (\textit{$^{\circ}$}) & 0, 90, 180, 270 & 0, 90, 180, 270 & 0, 90, 180, 270\\
 		\hline
  		row disp. (\textit{m}) & \textpm0.5, \textpm0.3, \textpm0.1 & \textpm0.4, \textpm0.2, 0 & \textpm0.4, \textpm0.2, 0\\
 		\hline 
 		col disp. (\textit{m}) & \textpm0.5, \textpm0.3, \textpm0.1 & \textpm0.5, \textpm0.3, \textpm0.1 & \textpm0.5, \textpm0.3, \textpm0.1 \\
 		\hline
		\end{tabular}}
	\end{center}
\caption{\textit{Map generation parameters}: The interpolation test parameters have parameters that interpolate in between the training parameters. The extrapolation test parameters are the same as the interpolation, except that the obstacle lengths are longer. }
\label{table:map_generation_parameters}
\vspace*{-0.02in}
\end{table}
 \subsection{Expert Planner}
 We use the $A^*$ algorithm to generate labels.
 %%TODO COMPLETE THIS
 
 \subsection{Neural Networks}
 We evaluate four separate neural network architectures: FF, LSTM, DNC FF, and DNC LSTM. The inputs at each time step are the $1080$-dimensional LIDAR reading $z_{t}$, and the $2$-dimensional position vector $(\mathsf{x}_t - \mathsf{x}_t^{g} ,\mathsf{y}_t - \mathsf{y}_t^{g})^T$ representing the displacement between the robot and the goal. Please see Fig. \ref{fig:network_architectures} for the network architectures.
 
The LIDAR is processed through 2 convolutional layers before being combined with the other inputs in the first fully connected layer. The convolution first convolution kernel is size $[10, 1, 10]$ with a stride of $10$. The second convolution kernel is size $[10, 10, 32]$ with a stride of $10$.

For the LSTM models, the LSTM hidden state has dimension $256$. The memory matrix (indicated in purple) is size $256 \mathsf{x} 64$ and has $4$ read heads and $1$ write head.

The last upstream layer (indicated in green) for all $4$ models has dimension $256$. The linear readout layer (indicated in red) outputs a $4$ dimensional action vector. 

\subsection{Training Implementation}
The Asynchronous DAgger algorithm is used to train the neural networks. For the two feedforward networks, the training batch size is $5$. For the two recurrent networks, the BPTT algorithm is truncated at $5$ steps. We use the RMSProp \cite{tieleman2012lecture} optimization algorithm with a learning rate of $10^{-4}$ to calculate the gradient.

Our learning algorithm is implemented in python using TensorFlow \cite{tensorflow2015-whitepaper}. Due to the python global interpreter lock (GIL), multithreading in python will not work well. As a result, our simulation environment and $A^*$ planning algorithm are implemented in C++, and we interface with Python using PyBind11. This allows us to release the GIL before any long-running executions in our C++ code (calling TensorFlow session runs also releases the GIL) and achieves good multi-threading performance. We train on a 16-core CPU with $32$ parallel learners.



==> tex/MapDifficulty.tex <==
\section{Map Difficulty}
\label{sec:mapdifficulty}

\subsection{Defining map difficulty}

A generalized notion of map difficulty is not easy to define. Most approaches define the idea of difficulty or complexity in terms of specific planning algorithms, rather than in terms of maps. The most similar concept to map difficulty is computational complexity of specific planning algorithms \cite{karaman2010incremental}\cite{choudhury2015theoretical}. However these definitions do not capture map difficulty since they ignore the map configuration, and instead relate complexity in terms of the planning algorithm and planning resolution. 

One possible definition for map difficulty is the number of expanded nodes searched for in the $A^{*}$ planner. The larger the number of expanded nodes, the more difficult it is for $A^*$ to find the path. Although this definition is limited to the $A^{*}$ planner, we use this definition in our experiments since our networks are trained in a supervised manner using $A^{*}$ to generate the labels. Specifically, our environments consist of cul-de-sac obstacles, so we define the difficulty of our maps by the obstacle length $l$. 

\subsection{Interpolation vs. Extrapolation}

We compare the separability and generalizability of the network architectures by using both the training and testing data. We evaluate separability using the training error, and additionally demonstrate a method to estimate the VC dimension. We then compare these VC dimension estimates to actual generalization performance on held-out interpolation and extrapolation test sets. The interpolation test set contains unseen maps with obstacle lengths that are interpolated between the training set obstacle lengths. The extrapolation test set contains obstacle lengths that are longer than those seen in the training set, and is more difficult both because the map difficulty is higher, and also because extrapolation is challenging.

\subsection{Blind navigation}

We test the ability of the network architectures by limiting the field of view of the lidar scan. Specifically, we prevent our networks from observing obstacles behind it, and force them to rely on memory while backtracking out of the cul-de-sac. This blind backtracking makes the navigation problem more difficult, but is not captured by map dependent $l$.








